Horizontal Scaling of Transaction-Creating Machines

Blockchain technology has become one of the most popular trends in IT over the last few years. Its increasing popularity and the discovery of ever more use cases raises the question of how to improve scalability. While researchers are exploring ways to scale the on-chain processing of transactions, the scalability of the off-chain creation of transactions has not been investigated yet. This is relevant for organizations wishing to send a high volume of transactions in a short time frame, or continuously, e.g., manufacturers of high-volume products. Especially for blockchain implementations such as Ethereum, which require transactions to include so-called nonces (essentially a sequence number), horizontally scaling transaction creation is non-trivial. In this paper, we propose four different approaches for horizontal scaling of transaction creation in Ethereum. Our experimental evaluation examines the performance of the different approaches in terms of scalability and latency and finds two of the four proposed approaches feasible to scale transaction creation horizontally.

==> Rebuttal.tex <==
Thanks to all reviewers for their comments and input. We focus the rebuttal on the clarification of the major aspects mentioned in the reviews.

R1:
- References/literature: we will conduct another careful literature search, and aim to include more recent related literature in the paper. If the reviewers have any specific pointers to literature that they feel we should discuss, we would be very grateful for those.
- Errors: we will conduct a careful proof read and use additional grammar-checking tools.
- Contribution: we will formulate a new paragraph in the introduction to further highlight the contribution and make it explicit.
- Additional improvements: We totally agree with this comment. In future work, the performance can likely be improved further, and mechanisms for increasing robustness should be investigated. 
Given that this is the first paper on the topic, we believe a number of improvements and additional aspects will be addressed by us and other researchers in the future. We will edit the conclusion section to highlight these aspects.

R2: Thanks a lot for highlighting unclear sections.
The reviewer asked: "Can you please highlight how, in your simulation, one VM for simulating private Ethereum n/w could handle so many transactions, but you need multiple tx creating machines?" In response, we want to raise three points:
- First, regarding "in your simulation": we performed an experimental evaluation, with actual code that is available for download, see Footnote 5; hence, replication of the experiments should be possible. The reviewer's comment shows that we need to formulate the evaluation method more clearly, thanks. We will reformulate the entire start of Section 4 accordingly.
- Second, we did not provide all details of the blockchain node in the paper, which we will fix in Section 4. Our node ran Geth with PoA, 400M gas per block, 1 block every 5 sec -> theoretically up to ~3800 tps would be possible in this configuration. We will run an experiment to determine the actual max. throughput in the setting chosen.
- Third, why one VM for the blockchain was sufficient: it appears that creating and signing txs is a computationally much more expensive task than verifying signatures and creating blocks in PoA. We will amend the description of the experimental setup and the discussion to address this point (Sections 4 & 5).

- As for the other comment: we absolutely agree that Approach 1 has its weaknesses, and it is obvious that it would not scale well once capacity of the middleware is reached. However, when and where these downsides become relevant (how many machines, how many tps?) was unclear and unknown before our analysis, and hence an interesting set of initial questions arose from Approach 1. We discuss its limitations at the end of Section 3.1 and the beginning of Section 5, and will revisit the discussion to explain the rationale for including this approach.

R3:
- Thanks for the assessment and suggested improvements, which we will implement.
